Non-Normal Modal Description Logics (Extended Version)

Modal logics are widely used in multi-agent systems to reason about actions, abilities, norms, or epistemic states. Combined with description logic languages, they are also a powerful tool to formalise modal aspects of ontology-based reasoning over an object domain. However, the standard relational semantics for modalities is known to validate principles deemed problematic in agency, deontic, or epistemic applications. To overcome these difficulties, weaker systems of so-called non-normal modal logics, equipped with neighbourhood semantics that generalise the relational one, have been investigated both at the propositional and at the description logic level. We present here a family of non-normal modal description logics, obtained by extending ALC-based languages with non-normal modal operators. For formulas interpreted on neighbourhood models over varying domains, we provide a modular framework of terminating, correct, and complete tableau-based satisfiability checking algorithms in NExpTime. For a subset of these systems, we also consider a reduction to satisfiability on constant domain relational models. Moreover, we investigate the satisfiability problem in fragments obtained by disallowing the application of modal operators to description logic concepts, providing tight ExpTime complexity results.

==> sec_app_coal.tex <==
\section{Description Logics of Agency and Ability}


\subsection{DL extension of Elgesem's logic}

\subsubsection{Syntax}


An $AL^{n}_{\ALC}$ \emph{concept} is an expression of the form
\[
C ::= A \mid \lnot C \mid C \sqcap C \mid \exists \role.C \mid \mathbb{B}_{i} C \mid \mathbb{C}_{i} C,
\]
where $A \in \NC$, $\role \in \NR$, while $\mathbb{B}_{i}$ and $\mathbb{C}_{i}$, with
$i \in J = \{ 1, \ldots, n \}$,
are \emph{agency} and \emph{ability} \emph{modalities}, respectively.

An \emph{$AL^{n}_{\ALC}$ formula}
takes the form
\[
\p ::= \pi \mid \neg \p \mid \p \land \p \mid \mathbb{B}_{i} \p \mid \mathbb{C}_{i} \p,
\]
where
$\pi$ is an $AL^{n}_{\ALC}$ atom
and
$i \in J$.





\subsubsection{Semantics}


An \emph{agency neighbourhood frame}, or simply \emph{frame}, is a pair $\Fmc = ( \Wmc, \{\Nmc^{\mathbb{B}}_i , \Nmc^{\mathbb{C}}_i \}_{i \in J})$,
where $\Wmc$ is a non-empty set of worlds and, for each $i \in J = \{1, \ldots, n\}$, $\Nmc^{\mathbb{B}}_{i}$ and $\Nmc^{\mathbb{C}}_{i}$ are neighbourhood functions satisfying the following conditions, for every
$i \in J$, $w \in \Wmc$, and $\alpha, \beta \subseteq \Wmc$:
%
\begin{itemize}
	\item $\Wmc \not \in \Nmc^{\mathbb{C}}_i(w)$;
	\item $\emptyset \not \in \Nmc^{\mathbb{C}}_i(w)$;
	\item if $\alpha\in \Nmc^{\mathbb{B}}_i(w)$ and $\beta\in \Nmc^{\mathbb{B}}_i(w)$, then $\alpha\cap\beta\in \Nmc^{\mathbb{B}}_i(w)$;
	\item if $\alpha \in \Nmc^{\mathbb{B}}_i(w)$, then $w \in \alpha$;
	\item $ \Nmc^{\mathbb{B}}_i(w) \subseteq  \Nmc^{\mathbb{C}}_i(w)$.
\end{itemize}

An \emph{$AL^{n}_{\ALC}$ varying} or \emph{constant domain neighbourhood model},
%or simply \emph{model},
based on an agency neighbourhood frame frame $\Fmc$, is a pair
$\Mmc = (\Fmc, \Int)$,
where
$\Fmc = (\Wmc, \{\Nmc^{\mathbb{B}}_{i}, \Nmc^{\mathbb{C}}_{i} \}_{i \in J})$ is an agency neighbourhood frame
and $\Imc$ is
defined as in Section~\ref{sec:prelim}, for the case of varying or constant domain neighbourhood models, respectively.
%a function
%associating with every $w \in \Wmc$ an \emph{$\ALC$ interpretation}
%$\Imc_{w} = (\Delta_{w}, \cdot^{\Imc_{w}})$,
%with non-empty \emph{domain} $\Delta_{w}$,
%and where $\cdot^{\Imc_{w}}$ is a function such that:
%for all $A \in \NC$, $A^{\Imc_{w}} \subseteq \Delta_{w}$;
%for all $\role \in \NR$, $\role^{\Imc_{w}} \subseteq \Delta_{w} {\times} \Delta_{w}$;
%for all $a \in \NI$, $a^{\Imc_{w}} \in \Delta$, and for all $u, v \in \reldomain$, $a^{\Imc_{u}}= a^{\Imc_{v}}$(denoted by $a^{\Imc}$).
%An \MLALC{n} \emph{constant domain neighbourhood model}
%is defined in the same way, except that, for all $w,w'\in\Wmc$,
%we have that $\Delta_{w}=\Delta_{w'}$.


\subsection{DL extension of Troquard's logic}


Given a finite set of \emph{agents} $J = \{ 1, \ldots, n \}$, we define $CL^{n}_{\ALC}$ \emph{concepts} and \emph{formulas} analogously to $AL^{n}_{\ALC}$, but with agency modalities $\mathbb{B}_{g}$ and ability modalities $\mathbb{C}_{g}$ indexed by a \emph{coalition} $g \subseteq J$.


A \emph{$CL^{n}_{\ALC}$ varying} or \emph{constant domain neighbourhood model} $\Mmc = (\Fmc, \Int)$ is defined analogously to the $AL^{n}_{\ALC}$ case, based on a \emph{coalitional agency neighbourhood frame} $\Fmc = ( \Wmc, \{\Nmc^{\mathbb{B}}_{g}, \Nmc^{\mathbb{C}}_{g} \}_{g \subseteq J})$.






==> sec_app_condom_frag.tex <==
\subsection{Proofs for Section~\ref{sec:fragcondom}}



\LemmapropE*
%
\begin{proof}
 If formula $\varphi$ is $\LnALCg$ satisfiable on constant domain neighbourhood models then, clearly,
$\prop{\varphi}$ is satisfied in a $\varphi$-consistent $L^{n}$ model.  
We now argue about the converse direction. 
Suppose $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $L^{n}$ model
$\propmodel = (\Wmc, \{ \Nmc_{i} \}_{i \in J}, \Vmc)$. 
We want to construct a constant domain neighbourhood model $\Mmc=(\Fmc,\Delta,\Imc)$, based on the $L^{n}$ frame $\Fmc = ( \Wmc, \{ \Nmc_{i} \}_{i \in J} )$, that satisfies 
$\varphi$.
%We define $\W$ as $\propdomain$ and \Nmc as $\propneigh$. 
%\todo{M: working here}
%The main point in this proof is the definition of \Imc and $\Delta$.
%
As $\propmodel$ is $\varphi$-consistent, for all $w\in \propdomain$,
\[
\alcform = \bigwedge_{p_{\elaxiom}\in \formtp{\varphi}} {\elaxiom} \ \wedge \bigwedge_{p_{\elaxiom} \in
\NPr(\varphi) \setminus \formtp{\varphi}}
% \overline{\NPr(w)}}
 \neg {\elaxiom},
\]
where
$\formtp{\varphi} = \{p_{\elaxiom} \in \NPr(\varphi) \mid w\in \Vmc(p_{\elaxiom})\}$,
%$$\formula(w) =  \bigwedge_{p_{\elaxiom}\in \NPr(w)} \hspace{-0.15cm} {\elaxiom} \ \wedge \hspace{-0.15cm} \bigwedge_{p_{\elaxiom}\in \overline{\NPr(w)}} \hspace{-0.15cm} \neg {\elaxiom}$$
is satisfied by an interpretation $\Jmc_{w}$.
It remains to argue that one can  define $\Imc$ 
where all $\Imc_{w}$ share the same domain $\Delta$ and 
the rigid individual name assumption holds (i.e., $a^{\Imc_{w}}=a^{\Imc_{v}}$, for all $w, v \in \W$ and all $a\in \NI$). 

By Lemma~\ref{lem:aux}, for each model $\Jmc_{w}$ of
$\alcform$
%$\formula(w)$
there is 
a quasimodel $\Qmc(w)$ for
$\alcform$.
%$\varphi$.
We denote by
$\Qmc_{\sf tp}(w)$ the set of concept types
  in  $\Qmc(w)$. 
We assume without loss of generality that
\begin{itemize}
\item[$(\ast)$] for all named types $t_a$, if $t_a\in\Qmc_{\sf tp}(w)$,
then $t=t_a\setminus\{a\}\in\Qmc_{\sf tp}(w)$.
\end{itemize}
We are now in position to define \Imc and $\Delta$. 
We define $\Delta$ as the set of functions $f: \W\rightarrow {\sf tp}(\varphi)$
such that (1) for all $w\in\W$, $f(w)\in \Qmc_{\sf tp}(w)$; and 
(2) $a\in f(w)$ iff $a\in f(u)$ for all $u,w\in \W$ and all $a\in \NI(\varphi)$.
By $(\ast)$ and the definition of $\Qmc_{\sf tp}(w)$,
we also have that (3) for all $w\in \W$ and all types $t\in\Qmc_{\sf tp}(w)$, 
there is $f\in\Delta$ such that $f(w)=t$. 
We denote by $f_a$ the unique element of $\Delta$ where $a$ occurs in it. 
For each $w\in \W$, we define the interpretation $\Imc_{w}$ as follows:
\begin{itemize}
\item for all $A\in\NC$, we have $f\in A^{\Imc_{w}}$ iff $A\in f(w)$;
\item for all $r\in\NR$, we have $(f,f')\in r^{\Imc_{w}}$ iff
$\{\neg D\mid \neg \exists r.D \in f(w)\}\subseteq f'(w)$.
\end{itemize}
Also, for all $w\in \W$ and all $a\in \NI(\varphi)$,
we require that $a^{\Imc_{w}}=f_a\in\Delta$ (for the other 
individual names the mapping is irrelevant for this proof, 
as long as it satisfies the rigid individual name assumption). 
By definition, $\Imc$ is a function mapping each $w\in\W$ to 
an interpretation $\Imc_{w}$ over the constant domain $\Delta$ and satisfying the %constraint 
rigid individual name assumption.

\todo{M: todo fix}
{\color{red}{
One can show that each $\Imc_{w}$ is a model of $\alcform$ using the fact that $\Qmc(w)$ is a quasimodel for $\alcform$. 
}}


{\color{blue}{
We first require the following result.

\todo{M: todo fix}
\begin{claim}\label{cl:localeq}
{\color{red}{
$\Jmc_{w} \models \alcform$ iff $\Imc_{w} \models \alcform$.
}}
\end{claim}
\begin{proof}
{\color{red}{\ldots}}
\end{proof}
}}

{\color{blue}{
Now, let $\Mmc=(\Fmc,\Delta,\Imc)$, with $\Fmc = ( \Wmc, \{ \Nmc_{i} \}_{i \in J} )$, $\Imc$, and $\Delta$ as defined above.
%By induction on the structure of subformulas $\psi$ of $\varphi$, we show
%in the following claim that,
%for every $w \in \Wmc$, we have
%$\propmodel, w \models \prop{\psi}$
%iff $\Mmc, w \models \psi$.
We now show the following claim.
 
\begin{claim}\label{cl:globaleq}
For every $\psi \in {\sf sub}(\varphi)$ and every $w \in \Wmc$, we have
$\propmodel, w \models \prop{\psi}$ iff
$\Mmc, w \models \psi$.
\end{claim}
\begin{proof}
The proof is by induction on the structure of subformulas $\psi$ of $\varphi$.
We first consider the base case.

\begin{itemize}
	\item $\psi = \pi$, where $\pi$ is an $\ALC$ atom in $\varphi$. Hence, $\prop{\psi} = p_\pi$, with $p_\pi$ propositional letter. By the semantics of propositional neighbourhood models,
$\propmodel, w \models p_{\pi}$ iff $w\in\Vmc(p_\pi)$. 
For every \ALC atom $\pi$ in $\varphi$, $w\in\Vmc(p_\pi)$ iff 
$\pi$ is a conjunct of $\hat{\varphi}_{\Vmc,w}$.
As $\propmodel$ is $\varphi$-consistent, we have that, for every $w\in \propdomain$,
the $\ALC$ formula
$\hat{\varphi}_{\Vmc,w}$
is satisfied by the $\ALC$ interpretation $\Jmc_{w} = (\Delta_{w}, \cdot^{\Jmc_{w}})$.
 Thus, $\pi$ is a conjunct of $\hat{\varphi}_{\Vmc,w}$ iff $\Jmc_w\models\pi$.
 \todo{AM: to fix, why?}
 {\color{red}{
 By
 Claim~\ref{cl:localeq},
% the semantics of $\MLnALCg$  neighbourhood models,
 }}
 the previous step is equivalent to
 $\Imc_w\models\pi$, i.e., $\Mmc, w \models \psi$.
 \end{itemize}
 For the inductive step, suppose that the claim holds for $\psi_1,\psi_2$. 
  We consider the following cases. 
 \begin{itemize}
 	\item $\psi=\neg\psi_1$: By the semantics of  propositional neighbourhood models,
 	$\propmodel, w \models \prop{\neg{\psi_1}}$ iff $\propmodel, w \not\models \prop{{\psi_1}}$. By the inductive hypothesis, Claim~\ref{cl:ind} holds for $\psi_1$.
 	By the contrapositive in each direction, $\propmodel, w \not\models \prop{{\psi_1}}$
 	iff $\Mmc, w \not\models \psi_1$. By the semantics of  $\MLnALCg$ neighbourhood models, $\Mmc, w \not\models \psi_1$ iff $\Mmc, w \models \neg\psi_1$.
\item $\psi=\psi_1\wedge\psi_2$: By the semantics of  propositional neighbourhood models,
$\propmodel, w \models \prop{{(\psi_1\wedge\psi_2)}}$ iff $\propmodel, w \models \prop{{\psi_1}}$ and $\propmodel, w \models \prop{{\psi_2}}$. By the inductive hypothesis, the claim holds for $\psi_1,\psi_2$.
So, $\propmodel, w \models \prop{{\psi_i}}$
iff $\Mmc, w \models \psi_i$, for $i\in \{1,2\}$. By the semantics of  $\MLnALCg$ neighbourhood models, $\Mmc, w \models \psi_1$ and $\Mmc, w \models \psi_2$ iff $\Mmc, w \models \psi_1\wedge \psi_2$.
\item $\psi=\B_{i} \psi_1$: By the semantics of  propositional neighbourhood models,
$\propmodel, w \models \prop{{(\B_{i} \psi_1)}}$ iff $\llbracket \prop{{\psi_1}}\rrbracket^{\propmodel} \in \Nmc_{i}(w)$ where
$\llbracket \prop{{\psi_1}} \rrbracket^{\propmodel} = \{ v \in \Wmc \mid \propmodel, v \models \prop{{\psi_1}} \}$. By the inductive hypothesis, the claim holds for $\psi_1$.
So, $\propmodel, v \models \prop{{\psi_1}}$
iff $\Mmc, v \models \psi_1$, for every $v\in\Wmc$. 
Thus, $\llbracket \prop{{\psi_1}} \rrbracket^{\propmodel}=\llbracket {{\psi_1}} \rrbracket^{\Mmc}$. By definition of $\propmodel$ and \Mmc, we have that $\Nmc_{i}(w)$
is the same in both $\propmodel$ and \Mmc, for every $w\in\Wmc$ and $i\in J$.
So $\llbracket \prop{{\psi_1}}\rrbracket^{\propmodel} \in \Nmc_{i}(w)$
iff $\llbracket {{\psi_1}} \rrbracket^{\Mmc} \in \Nmc_{i}(w)$.
By the semantics of  $\MLnALCg$ neighbourhood models, $\llbracket {{\psi_1}} \rrbracket^{\Mmc} \in \Nmc_{i}(w)$ iff $\Mmc, w \models \B_{i} \psi_1$.
 \end{itemize}
We have thus shown that for every subformula $\psi$ of $\varphi$ and every $w \in \Wmc$, we have
$\propmodel, w \models \prop{\psi}$ iff
$\Mmc, w \models \psi$.
\end{proof}
Since $\propmodel , v \models \prop{\varphi}$, for some $v \in \Wmc$, we conclude that $\varphi$ is $\LnALCg$ satisfiable. 
}}
\end{proof}


==> sec_fragcondom.tex <==
\subsection{Fragments without Modalised Concepts on Constant Domain}
\label{sec:fragcondom}
%\subsection{Satisfiability on Constant Domain for $\LnALCg$}
%\subsection{Satisfiability in Fragments without Modalised Concepts}




%\paragraph{Satisfiability in $\EALCg$  and $\MALCg$}
%\nb{O: working here}


\newcommand{\clf}{\ensuremath{{\sf sub}_{\sf f}}\xspace}
\newcommand{\clc}{\ensuremath{{\sf sub}_{\sf c}}\xspace}
\newcommand{\individuals}[1]{\ensuremath{\NI(#1)}\xspace}
In this section,
%the proof of Lemma~\ref{lem:propE}
we use the classical
notion of a quasimodel~\cite{GabEtAl03}, defined here for the convenience of the reader. 
{\color{blue}{
Let $\varphi$ be an \emph{$\ALC$ formula}, that is, an $\MLnALC$ formula without any occurrence of modal operators.
We assume without loss of generality that assertions occurring in $\varphi$ are of the form $A(a)$, where $A \in \NC$, or $r(a,b)$.
}}
We denote by $\NI(\formula)$ the set of individual names occurring in $\formula$. 
 Denote by $\clf(\formula)$ the closure under single negation of the set
of all formulas occurring in~$\formula$.  Similarly, we denote by
$\clc(\formula)$ the closure under single negation of the set of all
concepts union the concepts $A_{a}, \exists r.A_{a}$, for any
$a\in\individuals{\formula}$ and $r$ a role occurring in $\formula$,
where $A_a$ is a fresh concept name.
%As usual, the basic elements of our quasimodels are types.
%
A \emph{concept type for $\formula$} is any subset~$t$ of
$\clc(\formula)\cup\individuals{\formula}$ such that:
\begin{itemize}%[label=$\mathbf{T\arabic*}$,leftmargin=*]
  \item\label{ct:neg} $\neg C\in t$ iff $C\not\in t$, for all
    $\neg C\in\clc(\formula)$;
  \item\label{ct:con} $C\sqcap D\in t$ iff $C,D\in t$, for all
    $C\sqcap D\in\clc(\formula)$;
%    and
 \item\label{ct:ind} $t$ contains at most one individual name in~$\individuals{\formula}$.
\end{itemize}

\noindent
Similarly, we define \emph{formula types} $t\subseteq\clf(\formula)$ for $\formula$ with the
  conditions:
\begin{itemize}%[label=$\mathbf{T\arabic*'}$,leftmargin=*]
  \item\label{ft:neg} $\neg\psi\in t$ iff $\psi\not\in t$, for all
    $\neg\psi\in\clf(\formula)$;
%    and
  \item\label{ft:fcon} $\psi\wedge\chi\in t$ iff $\psi,\chi\in t$, for all
    $\psi\wedge\chi\in\clf(\formula)$.
\end{itemize}
We   omit `for $\formula$'  when there is no risk of confusion. 
%A concept type describes one domain element at a single time point,
%while a formula type expresses constraints on all domain elements.
%
If $a\in t\ \cap\ \individuals{\formula}$, then $t$ describes a named element. 
We  write $t_a$ to indicate this and call it a \emph{named type}.
%
%
We say that a pair of concept types $(t,t')$ is \emph{$r$-compatible} if
%\begin{align*}
$\{\neg F\mid \neg \exists
r.F\in t\}\subseteq t'.$ %\nb{A: changed E to F \\O: Ok!}
%\end{align*}
A \emph{quasimodel} for~$\formula$ is a set $\Qmc$ of concept or formula types for~$\formula$ 
such that:
\begin{itemize}%[label=\textbf{Q\arabic*},leftmargin=*]
  \item\label{q:fseg} $\Qmc$ contains exactly one formula type~$t_\Qmc$;
  \item\label{q:ind} $\Qmc$ contains exactly one named type $t_a$ for
    each $a\in\individuals{\formula}$;
  \item\label{q:gci} for all $C\sqsubseteq D\in\clf(\formula)$, we have
    $C\sqsubseteq D\in t_\Qmc$ iff $C\in t$ implies $D\in t$
    for all concept types $t \in \Qmc$;
  \item\label{q:cass} for all $A(a)\in\clf(\formula)$, we have
    $A(a)\in t_\Qmc$ iff $A\in t_a$ %\nb{A: changed C to A \\ O: Ok!};
    \item \label{q:quasi}   $t \in \Qmc$ and $\exists r.D \in t$ implies there is $t' \in \Qmc$
    such that $D\in t'$ and $(t,t')$ is      $r$-compatible;
    \item \label{q:last} for all $r(a,b)\in\clf(\formula)$, we have
      $r(a,b)\in t_\Qmc$ iff   
     $(t_a,t_b)$ is $r$-compatible. 
\end{itemize}
 
 

As usual, every quasimodel for~$\formula$ describes an  
interpretation satisfying~$\formula$ and, conversely,   every such interpretation can be 
abstracted into a quasimodel for~$\formula$. We formalise the correspondence 
between models and quasimodels  with 
the following lemma. 

%\nb{TODO define quasimodel as in yellow but with ind names in concept types, define types}
\begin{lemma}\label{lem:aux}
There is a quasimodel for an \ALC formula   iff 
there is a model of it. 
\end{lemma}

%We are now ready for proving Lemma~\ref{lem:propE}.
We now formalise the connection between %complexity of 
the satisfiability problem for 
$\LnALCg$ formulas on constant domain neighbourhood models and their propositional abstractions %with consistent models
with the following lemma.
%, which is an adaptation of the 
%results obtained for other \ALC extensions~\cite{Baader:2012:LOD:2287718.2287721}.
%~ %We say that a model of $\prop{\varphi}$
%~ %is $\varphi$-consistent

%\nb{$\varphi$-consistent model}

\begin{restatable}{lemma}{LemmapropE}\label{lem:propE}
\nb{M: todo fix proof}
A
%$\MLnALCg$
formula $\varphi$ is
$\LnALCg$
satisfiable
on constant domain neighbourhood models
iff
$\prop{\varphi}$ is satisfied in a $\varphi$-consistent $L^{n}$ model.
%A formula $\varphi$ is $\EALCg$ satisfiable
%iff
%%if, and only if, 
%$\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\E^{n}$ model.  
\end{restatable}
%


We can now use again to Lemma~\ref{lem:proplemmaL} to  characterise satisfiability of  $\prop{\varphi}$ in a $\varphi$-consistent model by the existence of a  $\varphi$-consistent valuation satisfying suitable corresponding properties.
%
%
%We
%%\nb{M: moved footnote here to save space}
%%\nb{M: todo fix notation}
%assume that the 
%primitive
%%propositional
%connectives used to build 
%%the
%propositional formulas are $\neg$ %, $\vee$, 
%and $\wedge$ ($\vee$ is expressed using 
%$\neg$ %, $\vee$, 
%and $\wedge$),
%%Moreover,
%and
%we
%denote by  ${\sf sub}(\prop{\varphi})$ the set 
%of subformulas of $\prop{\varphi}$ closed under single negation.  
%A \emph{valuation} for a propositional
%$\MLn$
%%modal logic
%formula $\prop{\varphi}$   
%is a function $\nu: {\sf sub} (\prop{\varphi})\rightarrow \{0,1\}$ that 
%satisfies the following conditions:
%%\footnote{Assuming that the 
%%primitive propositional connectives used to build 
%%the formulas are $\neg$ %, $\vee$, 
%%and $\wedge$ ($\vee$ is expressed using 
%%$\neg$ %, $\vee$, 
%%and $\wedge$).}:
%(1) for all $\neg\psi\in {\sf sub} (\prop{\varphi})$,
%$\nu(\psi)=1$ iff $\nu(\neg\psi)=0$;
%%(2) for all $\psi_1\vee \psi_2\in {\sf sub} (\prop{\varphi})$,
%%$\nu(\psi_1\vee \psi_2) = 1$ iff $\nu(\psi_1) = 1$
%%or $\nu(\psi_2) = 1$; 
%(2) for all $\psi_1\wedge \psi_2\in {\sf sub} (\prop{\varphi})$,
%$\nu(\psi_1\wedge \psi_2) = 1$ iff $\nu(\psi_1) = 1$
%and $\nu(\psi_2) = 1$; 
%and (3) $\nu(\prop{\varphi})=1$. 
%We say that a valuation for $\prop{\varphi}$ 
%is \emph{$\varphi$-consistent} if any %propositional
%neighbourhood model of the form $(\{w\}, \{ \propneigh_{i} \}_{i \in [1, n]}, \propassign)$ satisfying
%$w\in \propassign(p_\elaxiom)$ iff $\nu(p_\elaxiom)=1$, for all $p_\elaxiom\in \NPr(\varphi)$, 
% is $\varphi$-consistent.
%We now establish that satisfiability of 
%$\prop{\varphi}$ in a $\varphi$-consistent model is characterized 
%by the existence of a  $\varphi$-consistent valuation 
%satisfying the property described in Lemma~\ref{lem:propsat}.
%%
%\begin{restatable}{lemma}{Lemmapropsat}\label{lem:propsat}
%A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\E^{n}$ model
%iff
%%if, and only if,
%there is   a $\varphi$-consistent valuation \valuation 
%for $\prop{\varphi}$ such that if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%$\valuation(\B_i\psi_2)=0$, then $(\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$
%is satisfied in a $\varphi$-consistent $\E^{n}$ model. 
%\end{restatable}
%%
% \begin{proof}
% ($\Rightarrow$) Suppose that $\prop{\varphi}$ is satisfied in a world $w$ of a $\varphi$-consistent model 
% $\propmodel = (\propdomain, \{ \propneigh_{i} \}_{i \in [1,n]}, \propassign)$. That is, 
% $\propmodel, w\models \varphi$. We define a $\varphi$-consistent valuation for 
% $\prop{\varphi}$
% by setting $\nu(\psi)=1$ if $\propmodel, w\models \psi$ and $\nu(\psi) = 0$
% if  $\propmodel, w\not\models \psi$. 
% It is easy to check that $\nu$ is indeed a 
% $\varphi$-consistent valuation (given that $\propmodel$ is 
% $\varphi$-consistent). Assume that 
% $\B_i\psi_1$ and $\B_i\psi_2$ are in ${\sf sub}(\prop{\varphi})$, 
% $\nu(\B_i\psi_1)=1$ and $\nu(\B_i\psi_2)=0$. Then $\propmodel,w\models \B_i\psi_1$
% and $\propmodel,w\not\models \B_i\psi_2$. Thus, by definition, 
% $\propassign(\psi_1)\in \propneigh_i(w)$ and 
%  $\propassign(\psi_2)\not\in \propneigh_i(w)$.
%%Using the same argument of Lemma 3.1 in~\cite{Var2}, it follows that 
%So,
%   $\propassign(\psi_1)\neq \propassign(\psi_2)$.
%Then %it is easy to see that
% there 
%   is a world $u$ in the symmetrical difference of these sets 
%   such that $\propmodel,u\models (\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$. 
%   
% ($\Leftarrow$) Suppose there is a $\varphi$-consistent valuation $\nu$ for $\prop{\varphi}$ such that 
% if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%$\valuation(\B_i\psi_2)=0$, then 
%there is a $\varphi$-consistent model \[\propmodel_{\psi_1,\psi_2}=(\propdomain_{\psi_1,\psi_2},
%\{ \propneigh_{{\psi_1,\psi_2}_{i}} \}_{i \in [1,n]},\propassign_{\psi_1,\psi_2})\]
% and a world 
%$w_{\psi_1,\psi_2}\in \propdomain_{\psi_1,\psi_2}$ such that 
%$\propmodel_{\psi_1,\psi_2}, w_{\psi_1,\psi_2}\models (\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$. 
%
%Let $\propmodel_1,\ldots,\propmodel_m$ be an enumeration of the models 
%$\propmodel_{\psi_1,\psi_2}$, as above.  That is, we take one model for each 
%pair $\psi_1,\psi_2$ where $\propmodel_j = (\propdomain_j, \{ \propneigh_{j_{i}} \}_{i \in [1,n]},\propassign_j)$, 
%and let $w_1,\ldots,w_m$ be an enumeration of the worlds $w_{\psi_1,\psi_2}$, 
%with $w_j\in \propdomain_j$. We assume w.l.o.g. that $\propdomain_j\cap \propdomain_k=\emptyset$ 
%for $j\neq k$. 
%
%In the following, we define a $\varphi$-consistent  model   $\propmodel = (\propdomain,\{ \propneigh_{i} \}_{i \in [1,n]}, \propassign)$ 
%for $\prop{\varphi}$. 
%Intuitively, we construct $\propmodel$ by taking the union of each 
%$\propmodel_j$ with the addition of a new world $w$ that 
%will satisfy $\prop{\varphi}$. 
%We define $\propdomain$ as $\bigcup_{1\leq j\leq n}\propdomain_j\cup \{w\}$, 
%where $w$ is fresh.
%%The tricky part of the proof is to define the assignment $\propassign$. 
%Before defining $\propneigh_{i}$ and $\propassign$, we define the function $J: {\sf sub}(\prop{\varphi})\rightarrow \Pmc(\Wmc)$
%with $J(\psi)=\bigcup_{0\leq j \leq m} \Vmc_j(\psi)$ for all $\psi\in {\sf sub}(\prop{\varphi})$, where %$I_i$ is as above for $1\leq i\leq n$, 
% %and
%$\Vmc_0: {\sf sub}(\varphi)\rightarrow  \Pmc(\{w\})$ is the function
%that assigns $\psi$ to $\{w\}$, if $\nu(\psi)=1$, 
%and to $\emptyset$, otherwise ($\Vmc_j$, for $1\leq j\leq m$, is as above).
%By construction, we have that $J(\neg \psi)=\propdomain\setminus J(\psi)$
%and $J(\psi_1\wedge \psi_2)=J(\psi_1)\cap J(\psi_2)$. 
%We define the assignment $\propassign$ as the function 
%$\propassign: \NPr(\varphi)\rightarrow \Pmc(\Wmc)$ satisfying 
% $\propassign(p_\elaxiom)=J(p_\elaxiom)$ for all $p_\elaxiom\in \NPr(\varphi)$. 
% 
%It remains to define $\propneigh_i$, for $1 \leq i \leq n$. 
%For $u\in \propdomain_j$ and $\B_i\psi \in {\sf sub}(\varphi)$, we   put $J(\psi) \subseteq \Wmc$ in $\propneigh_i(u)$ 
%precisely when $\propmodel_j,u \models \B_i \psi$.  
%%and $\alpha = J(\psi_\alpha)$
%%for some $\B_i\psi_\alpha \in {\sf sub}(\varphi)$.
%We claim that 
%if $\beta \in \Nmc_i(u)$ and $\beta = J(\psi)$ for some $\B_i\psi\in{\sf sub}(\prop{\varphi})$,
%then $\propmodel_j,u\models\B_i\psi$.
%Indeed, since $\beta = J(\psi)\in \Nmc_i(u)$, 
%we must have that $\propmodel_j,u\models \B_i\psi_{\beta}$ and  $\beta = J(\psi_{\beta})$ for 
%some $\B_i\psi_\beta \in{\sf sub}(\prop{\varphi})$.
%But since
%$J(\psi)=J(\psi_\beta)$, we also have $\propassign_j(\psi)=\propassign_j(\psi_\beta)$ 
%(recall that $\propdomain_j \cap \propdomain_k = \emptyset$ for  
%$k \neq j$), so $\propmodel_j,u\models \B_i\psi$ iff 
%$\propmodel_j,u \models \B_i \psi_\beta$.
%It follows that $\propmodel_j,u\models \B_i\psi$.
%
%Also, we put $\alpha \subseteq \Wmc$ in $\propneigh_i(w)$ (recall $w$ is the fresh 
%world introduced above in $\propdomain$) precisely 
%when $\nu(\B_i\psi_\alpha) = 1$ and $\alpha = J(\psi_\alpha)$ for some 
%$\B_i\psi_\alpha \in {\sf sub}(\prop{\varphi})$.
%We claim that if 
%$\beta \in \propneigh_i(w)$ and $\beta = J(\psi)$ for some $\B_i \psi \in{\sf sub}(\prop{\varphi})$ 
%then $\nu(\B_i \psi) = 1$.
%Indeed, since $\beta = J(\psi)\in \propneigh_i(u)$ 
%we must have that $\nu(\B_i\psi_\beta)=1$ and $\beta = J(\psi_\beta)$ for some 
%$\B_i\psi_\beta \in{\sf sub}(\prop{\varphi})$. 
%Suppose now that $\nu(\B_i\psi) = 0$. Then, by assumption, there exists a structure
%$\propmodel_j = (\propdomain_j, \{ \propneigh_{j_i} \}_{i \in [1, n]}, \propassign_j)$ and a world $w_j
%\in \propdomain_j$ such that $\propmodel_j,w_j \models (\psi_\beta \wedge \neg\psi)\vee(\neg\psi_\beta \wedge \psi)$. 
%It follows that $\propassign_j(\psi_\beta)\neq \propassign_j(\psi)$. 
%Consequently $J(\psi_\beta)\neq J(\psi)$, which is a contradiction.  
%%\nb{O :... talk about consistent}
%
%We now show by induction on the structure of formulas 
%that $\propassign$ and $J$ agree on ${\sf sub}(\prop{\varphi})$. 
%This holds by construction for atomic propositions. It is easy to deal 
%with propositional connectives, since we know that $J(\neg \psi)=\propdomain\setminus J(\neg \psi)$
%and  $J(\psi_1\wedge \psi_2)=J(\psi_1)\cap J(\psi_2)$ 
%and similarly for $\propassign$. Assume inductively that $\propassign(\psi) = J(\psi)$.
%Suppose first that $u\in J(\B_i\psi)$. Then, either $u=w$ and $\nu(\B_i\psi)=1$
%or $u\in \propdomain_j$ and $\propmodel_j,u\models\B_i\psi$. In either case 
%we have that $J(\psi)\in \propneigh_i(u)$. Since 
%$\propassign(\psi) = J(\psi)$, it follows that $\propmodel,u\models \B_i\psi$, 
%that is, $u\in \propassign(\B_i\psi)$. Suppose now that $u\in \propassign(\B_i\psi)$, 
%that is, $\propmodel,u\models \B_i\psi$, or, equivalently, $\propassign(\psi)\in \propneigh_i(u)$.
%Since $\propassign(\psi) = J(\psi)$ it follows that either $u=w$ and 
%$\nu(\B_i\psi)=1$ or $u\in \propdomain_j$ and $\propmodel_j,u\models \B_i\psi$. 
%In either case we have that $u\in J(\B_i\psi)$. 
%
%Since $\nu(\prop{\varphi})=1$, we have that $w\in J(\prop{\varphi})$, 
%and consequently $w\in \propassign(\prop{\varphi})$. That 
%is, $\propmodel,w\models\prop{\varphi}$. 
%The fact that $\propmodel$ is $\varphi$-consistent follows from 
%the fact that $\nu$, used to construct the assignment 
%related to $w$, is $\varphi$-consistent and 
%the models $\propmodel_1,\ldots,\propmodel_m$, used to define 
%the remaining worlds in $\Wmc$, are all $\varphi$-consistent. 
%\end{proof}
%
Finally, to check satisfiability of $\prop{\varphi}$ in a $\varphi$-consistent model, we \ldots
%use Lemma~\ref{lem:propsat} and the fact that
%there are only quadratically many formulas of the form $\psi_1\wedge\neg\psi_2$, 
%where $\psi_1$ and $\psi_2$ are subformulas of $\prop{\varphi}$. 
%We observe that satisfiability in \ALC is \ExpTime-complete~\cite{GabEtAl03}
%and so, one can determine in exponential 
%time whether a valuation is $\varphi$-consistent.
%For an $\ExpTime$ upper bound, one can deterministically compute 
%all possible $\varphi$-consistent valuations for $\psi_1\wedge\neg\psi_2$ 
%and decide satisfiability of $\prop{\varphi}$ by a $\varphi$-consistent
%model using a bottom-up strategy (as in~\cite{Var2}). 
%As satisfiability in \ALC 
%is \ExpTime-hard  our upper bound is tight.
This leads us to the following tight complexity result.

\begin{restatable}{theorem}{Theorempropsat}\label{thm:propsat}
The $\LnALCg$ formula satisfiability problem on constant domain neighbourhood models is $\ExpTime$-complete.
\end{restatable}

%To determine satisfiability of $\prop{\varphi}$ in a $\varphi$-consistent
%model, we use Lemma~\ref{lem:propsat} and the fact that
%there are only quadratically many formulas of the form $\psi_1\wedge\neg\psi_2$, 
%where $\psi_1$ and $\psi_2$ are subformulas of $\prop{\varphi}$. 
%We observe that satisfiability in \ALC is \ExpTime-complete~\cite{GabEtAl03}
%%~\cite{dlhandbook},
%%\nb{M: Changed ref. to shrink bib} 
%and so, one can determine in exponential 
%time whether a valuation is $\varphi$-consistent.
%For an $\ExpTime$ upper bound, one can deterministically compute 
%all possible $\varphi$-consistent valuations for $\psi_1\wedge\neg\psi_2$ 
%and decide satisfiability of $\prop{\varphi}$ by a $\varphi$-consistent
%model using a bottom-up strategy (as in~\cite{Var2}). 
%As satisfiability in \ALC 
%%and in the propositional modal logic \E{} 
%is \ExpTime-hard  our upper bound is tight.
%
%\begin{restatable}{theorem}{Theorempropsat}\label{thm:propsat}
%The $\EALCg$ formula satisfiability problem on constant domain neighbourhood models is $\ExpTime$-complete.
%\end{restatable}

%Regarding the proof for \MALCg, we first point out that 
%Lemma~\ref{lem:propE} can be easily adapted to \MALCg. 
%%the proof for the propositional case $\Mn^n$~\cite{Var2} can be similarly 
%%adapted to our combination with \ALC.
%%~ Lemma~\ref{lem:prop} can be easily adapted to \MALCg. 
%%~ We now formalize a variant of Lemma~\ref{lem:propsat} 
%%~ for \MALCg. 
%%We   establish a variant of Lemma~\ref{lem:propsat} 
%%tailored for $\Mn^{n}$ (see Proposition 3.8 in~\cite{Var2}).
%The proof for our $\ExpTime$ result for \MALCg 
%is analogous to the one given for \EALCg, except that here  we use 
%a variant of 
%%the following variant of
%Lemma~\ref{lem:propsat} 
%tailored for $\EM^{n}$
%%\nb{M: todo fix}
%(see Proposition 3.8 in~\cite{Var2}).
%%Lemma~\ref{lem:propsatm} and an adaptation of Lemma~\ref{lem:prop}.
%%\begin{restatable}{lemma}{Lemmapropsatm}\label{lem:propsatm}
%%A formula $\prop{\varphi}$ is $\Mn^{n}$ satisfiable by a $\varphi$-consistent model
%%if, and only if, there is   a $\varphi$-consistent valuation \valuation 
%%for $\prop{\varphi}$ such that if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%%$\valuation(\B_i\psi_2)=0$, then $\psi_1\wedge\neg\psi_2$
%%is $\Mn^{n}$ satisfiable by a $\varphi$-consistent model. 
%%\end{restatable}
%%the proof for the propositional case $\Mn^n$~\cite{Var2} can be similarly 
%%adapted to our combination with \ALC. 
%Thus, we obtain also the following result.
%%\nb{M: changed a bit. Do you prefer the previous sentence? Fine with me}
%%We are now ready for Theorem~\ref{thm:propsat}. 
%\begin{restatable}{theorem}{Theorempropsat}\label{thm:propsat}
%The $\MALCg$ formula satisfiability problem on constant domain neighbourhood models is $\ExpTime$-complete.
%%Satisfiability  in \MALCg %and \EEL{g} 
%% is \ExpTime-complete.
% % and 
%%\NP-complete, respectively. 
%\end{restatable}
%
%%~ Regarding \MALCg, the proof for the propositional case $\Mn^n$~\cite{Var2} can be similarly 
%%~ adapted to our combination with \ALC. 
%
%%~ \begin{restatable}{theorem}{Theorempropsat}\label{thm:propsat}
%%~ Satisfiability  in \MALCg %and \EEL{g} 
% %~ is \ExpTime-complete.
% %~ % and 
%%~ %\NP-complete, respectively. 
%%~ \end{restatable}
%
%%\paragraph{{\color{red}{M: $\ExpTime$-completeness of $\EALCg$ (and $\MALCg$, analogously)}}}
%%(Sketch, cf.~\cite{Baader:2012:LOD:2287718.2287721})
%%\nb{M: Check!}
%%
%%\medskip
%%\noindent
%%Upper bound:
%%
%%\medskip
%%1 -- Given a $\MLALC{}$ formula $\p$, compute its propositional abstraction $\prop{\p}$.
%%
%%\medskip
%%2 -- Define:
%%\[
%%S := \{ X_1, \ldots, X_k \} \subseteq \NPr(\{ p_1, \ldots, p_n \})
%%\]
%%\[
%%\p_{X_{i}} := (\bigwedge_{p_{j} \in X_{i}} \pi_{j} \land \bigwedge_{p_{j} \not \in X_{i}} \pi_{j} );
%%\qquad
%%\p_{X} := \bigwedge_{1 \leq i \leq k} \p_{X_{i}}
%%\]
%%\[
%%\prop{\p}^{S} := \prop{\p} \land \bigwedge_{1 \leq i \leq 3} \Box_{i} (\bigvee_{X \in S} (\bigwedge_{p \in X} p \land \bigwedge_{p \not \in X} p ))
%%\]
%%
%%\medskip
%%3 -- Prove:
%%
%%\begin{lemma}
%%A $\MLALC{3}^{g}$ formula $\p$ is satisfiable iff there is a set $S = \{ X_1, \ldots, X_k \} \subseteq \NPr(\{ p_1, \ldots, p_n \})$ such that the $\ML^{3}$ formula $\prop{\p}^{S}$ and the $\ALC$ formula $\p_{X}$ are satisfiable.
%%\end{lemma}
%%\begin{proof}
%%\end{proof}
%%
%%
%%\medskip
%%4 -- Define $S^{*}$ as the set of all subsets $X \subseteq \{p_1, \ldots, p_n \}$ such that the following $\ALC$ formula is satisfiable:
%%\[
%%\p_X := (\bigwedge_{p_{j} \in X} \pi_{j} \land \bigwedge_{p_{j} \not \in X} \pi_{j} )
%%\]
%%\[
%%\prop{\p}^{S^{*}} := \prop{\p} \land \bigwedge_{1 \leq i \leq 3} \Box_{i} (\bigvee_{X \in S^{*}} (\bigwedge_{p \in X} p \land \bigwedge_{p \not \in X} p ))
%%\]
%%
%%
%%\medskip
%%5 -- Prove:
%%
%%\begin{lemma}
%%Let $\p_1, \ldots, \p_k$ be $\ALC$ formulas over disjoint sets of individual, concept, and role names. Then $\p_1 \land \ldots \land \p_k$ is satisfiable iff, for each $i \in \{ 1, \ldots, k \}$, $\p_i$ is satisfiable.
%%\end{lemma}
%%\begin{proof}
%%\end{proof}
%%
%%\medskip
%%6 -- Prove:
%%\begin{lemma}
%%A $\MLALC{3}^g$ formula $\p$ is satisfiable iff the $\ML^{3}$ formula $\prop{\p}^{S^{*}}$ is satisfiable.
%%\end{lemma}
%%\begin{proof}
%%\end{proof}
%%
%%\medskip
%%7 -- Since computing $S^{*}$ and checking satisfiability of $\prop{\p}^{S^{*}}$ can be done in exponential time in the size of $\p$, using the translation $\cdot\tr$, we hae that the $\EALCg$ satisfiability problem is in $\ExpTime$.
%%
%%
%%\medskip
%%\noindent
%%Lower bound: from $\ExpTime$-hardness of $\ALC$.
%%
%%\begin{theorem}
%%The $\EALCg$ satisfiability problem is $\ExpTime$-complete.
%%\end{theorem}
%
%
%
%
%
%
%
%
%
%%\paragraph{Satisfiability in $\CALCg$  and $\NALCg$}
%%
%%In~\citeauthor{DL19}~\cite{DL19}, it is shown that 
%%$\EALCg$  and $\MALCg$ formula satisfiability problems on constant domain neighbourhood models are 
%%$\ExpTime$-complete.
%%
%We now show tight complexity results %$\ExpTime$ upper bounds 
%for $\CALCg$  and $\NALCg$,
%using again the notion of 
%a propositional abstraction of a formula 
%(as in, e.g.,~\cite{Baader:2012:LOD:2287718.2287721}).
%%Since $\ALC$ formula satisfiability is already $\ExpTime$-hard, 
%%our upper bounds here are tight. 
%%we have 
%%a tight complexity result for the global cases.
%%We show that
%Here, one can separate the satisfiability test into two parts, 
%one for the description logic dimension and 
%one for the 
%%dimension of the
%%\neighborhood
%%frame. 
%modal dimension.
%%~ In this subsection, we also consider the lightweight DL called \EL, defined 
%%~ as the fragment of \ALC which only allows conjunctions and existential quantification 
%%~ in concept expressions. 
%%
%%Consider $\Lmc\in\{\ALC,\EL\}$. 
%%\newcommand{\propmodel}{\ensuremath{M}\xspace}
%%\newcommand{\propdomain}{\ensuremath{W}\xspace}
%%\newcommand{\propneigh}{\ensuremath{N}\xspace}
%%\newcommand{\propassign}{\ensuremath{I}\xspace}
%The 
%\emph{propositional  abstraction} $\prop{\varphi}$ of an
%$\MLnALCg$
%%$\CALCg$ (respectively, $\NALCg$)
%formula $\varphi$ is  
%the result of replacing each $\ALC$
%CI
%%atom
%in $\varphi$ by 
%a propositional letter $p$, so that there is a $1:1$ relationship 
%between the $\ALC$
%CI
%%atoms
%$\elaxiom$ occurring in $\varphi$ and the 
%propositional letters $p_{\elaxiom}$ used for the abstraction.  
%%The semantics of $\prop{\varphi}$ is given in terms of \emph{propositional 
%%neighbourhood models} $ (\Wmc, \{ \Nmc_{i} \}_{i \in I}, \Vmc)$ for $\EC^{n}$ (respectively, $\EN^{n}$), 
%%where $(\Wmc, \{ \Nmc_{i} \}_{i \in I})$ is a neighbourhood frame 
%%and $\Vmc: \NPr \rightarrow 2^{\Wmc}$ is a function 
%%mapping propositional letters in $\NPr$ to
%%sets of worlds
%%%subsets of the domain of worlds
%%(see~\cite{Che,Var2}). 
%We set $\NPr(\varphi) = \{p_{\elaxiom}\in\NPr\mid \elaxiom \text{ is an \ALC
%CI
%%atom
%in }
%\varphi \}$.
%%
%Given an
%$\MLnALCg$
%%\nb{M: todo fix}
%%$\CALCg$ (respectively, $\NALCg$)
%formula $\varphi$, we say that a propositional neighbourhood model 
%$\propmodel = (\Wmc, \{ \Nmc_{i} \}_{i \in I}, \Vmc)$
%of $\prop{\varphi}$
%is \emph{$\consistent{\varphi}$}
%if, for all $w\in \Wmc$,
%the following \ALC formula is satisfiable $$\textstyle\bigwedge_{p_{\elaxiom}\in \NPr(w)} \ {\elaxiom} \ \wedge \
%\bigwedge_{p_{\elaxiom}\in \overline{\NPr(w)}}\ \neg {\elaxiom},$$
%where $\NPr(w) = \{p_{\elaxiom}\in \NPr(\varphi) \mid w\in \Vmc(p_{\elaxiom})\}$
%and $\overline{\NPr(w)}=\NPr(\varphi)\setminus\NPr(w)$. 
%We now formalise the connection between %complexity of the satisfiability problem for 
%$\MLnALCg$
%%$\CALCg$ and $\NALCg$
%formulas and their propositional abstractions %with consistent models
%with the following lemma, where $\mathit{L} \in \{ \EC, \EN \}$, obtained by adapting the proof of Lemma~\ref{lem:propE}
%%~\citeauthor{DL19}~\cite[Lemma~1]{DL19}.
%%, which is an adaptation of the 
%%results obtained for other \ALC extensions~\cite{Baader:2012:LOD:2287718.2287721}.
%%~ %We say that a model of $\prop{\varphi}$
%%~ %is $\varphi$-consistent
%
%%\nb{$\varphi$-consistent model}
%
%\begin{restatable}{lemma}{Lemmaprop}\label{lem:satfraglog}
%A formula $\varphi$ is $\LnALCg$ satisfiable
%on constant domain neighbourhood models
%iff
%%if, and only if, 
%$\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\mathit{L}^{n}$ model.  
%\end{restatable}
%
%%\begin{restatable}{lemma}{Lemmaprop}\label{lem:general}
%%A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent  
%%$\mathit{L}^{n}$
%%model
%%iff
%%if, and only if,
%%there is   a $\varphi$-consistent valuation \valuation 
%%for $\prop{\varphi}$ such that 
%%if $\B_i\psi_1,   \B_i\psi_2$ are in 
%%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$   and 
%%$\valuation(\B_i\psi_2)=0$, then either $(\psi_1\wedge\neg\psi_2)$ or 
%%$(\neg\psi_1\wedge\psi_2)$ 
%%is satisfied in a $\varphi$-consistent $\mathit{L}^{n}$
% %model. 
%%\begin{itemize}
%%\item if $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and
%%$\valuation(\B_i\psi_1)=0$ then $\neg \psi$ is 
%%$\EC^{n}$ satisfiable; and 
%%\item 
%%\end{itemize}
%%\end{restatable}
%
%We
%%\nb{M: moved footnote here to save space}
%%\nb{M: todo fix notation}
%assume that the 
%primitive
%%propositional
%connectives used to build 
%%the
%propositional formulas are $\neg$ %, $\vee$, 
%and $\wedge$ ($\vee$ is expressed using 
%$\neg$ %, $\vee$, 
%and $\wedge$),
%%Moreover,
%and
%we
%denote by  ${\sf sub}(\prop{\varphi})$ the set 
%of subformulas of $\prop{\varphi}$ closed under single negation.  
%A \emph{valuation} for a propositional
%$\MLn$
%%modal logic
%formula $\prop{\varphi}$   
%is a function $\nu: {\sf sub} (\prop{\varphi})\rightarrow \{0,1\}$ that 
%satisfies the following conditions:
%%\footnote{Assuming that the 
%%primitive propositional connectives used to build 
%%the formulas are $\neg$ %, $\vee$, 
%%and $\wedge$ ($\vee$ is expressed using 
%%$\neg$ %, $\vee$, 
%%and $\wedge$).}:
%(1) for all $\neg\psi\in {\sf sub} (\prop{\varphi})$,
%$\nu(\psi)=1$ iff $\nu(\neg\psi)=0$;
%%(2) for all $\psi_1\vee \psi_2\in {\sf sub} (\prop{\varphi})$,
%%$\nu(\psi_1\vee \psi_2) = 1$ iff $\nu(\psi_1) = 1$
%%or $\nu(\psi_2) = 1$; 
%(2) for all $\psi_1\wedge \psi_2\in {\sf sub} (\prop{\varphi})$,
%$\nu(\psi_1\wedge \psi_2) = 1$ iff $\nu(\psi_1) = 1$
%and $\nu(\psi_2) = 1$; 
%and (3) $\nu(\prop{\varphi})=1$. 
%We say that a valuation for $\prop{\varphi}$ 
%is \emph{$\varphi$-consistent} if any
%propositional
%neighbourhood
%model of the form $(\{w\}, \{ \propneigh_{i} \}_{i \in I}, \propassign)$ satisfying
%$w\in \propassign(p_\elaxiom)$ iff $\nu(p_\elaxiom)=1$, for all $p_\elaxiom\in \NPr(\varphi)$, 
% is $\varphi$-consistent.
%We now establish that satisfiability of 
%$\prop{\varphi}$ in a $\varphi$-consistent $\EC^{n}$ (respectively, $\EN^{n}$) model is characterized 
%by the existence of a  $\varphi$-consistent valuation 
%satisfying the property described in Lemma~\ref{lem:proplemma2} 
%(respectively, Lemma~\ref{lem:proplemmaN}).
%
%\begin{restatable}{lemma}{Lemmapropsec}\label{lem:proplemma2}
%A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\EC^{n}$ %\nb{check macro}
%model
%iff
%%if, and only if,
%there is   a $\varphi$-consistent valuation \valuation 
%for $\prop{\varphi}$ such that 
%if $\B_i\psi_1, \dots, \B_i\psi_k$ are in 
%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_j)=1$ for all $1\leq j < k$, and 
%$\valuation(\B_i\psi_k)=0$, then either $(\bigwedge^{k-1}_{j=1}\psi_j\wedge\neg\psi_k)$ or 
%$(\neg\psi_j\wedge\psi_k)$ for some $1\leq j < k$
%is satisfied in a $\varphi$-consistent $\EC^{n}$ %\nb{check macro}
% model. 
%%\begin{itemize}
%%\item if $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and
%%$\valuation(\B_i\psi_1)=0$ then $\neg \psi$ is 
%%$\EC^{n}$ satisfiable; and 
%%\item 
%%\end{itemize}
%\end{restatable}
%%
%\begin{proof}
%%\paragraph{Point 2}
%($\Rightarrow$) Suppose that $\prop{\varphi}$ is satisfied in a world $w$ of a $\varphi$-consistent $\EC^{n}$ model 
% $\propmodel = (\propdomain, \{ \propneigh_{i} \}_{i \in I}, \propassign)$. That is, 
% $\propmodel, w\models \prop{\varphi}$. We define a $\varphi$-consistent valuation for 
% $\prop{\varphi}$
% by setting $\nu(\psi)=1$ if $\propmodel, w\models \psi$ and $\nu(\psi) = 0$
% if  $\propmodel, w\not\models \psi$. 
% It is easy to check that $\nu$ is indeed a 
% $\varphi$-consistent valuation (given that $\propmodel$ is a  
% $\varphi$-consistent $\EC^{n}$ model). Assume  $\B_i\psi_1, \dots, \B_i\psi_k$ are in 
%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_j)=1$ for all $1\leq j < k$, and 
%$\valuation(\B_i\psi_k)=0$.
%%
%Then $\propmodel,w\models \B_i\psi_j$ for all $1\leq j < k$,
% and $\propmodel,w\not\models \B_i\psi_k$.
%By definition, $(\B_i \psi_1 \wedge \ldots \wedge \B_i \psi_{k-1})\rightarrow \B_i (\psi_1\wedge \ldots \wedge \psi_{k-1})$ holds in $\EC^{n}$ models.
%So $\propmodel,w\models \B_i (\psi_1\wedge \ldots \wedge \psi_{k-1})$ 
% and $\propmodel,w\not\models \B_i\psi_k$.
%This means that $\valuation(\B_i(\bigwedge^{k-1}_{j=1}\psi_j))=1$
%while $\valuation(\B_i\psi_k)=0$.
%  By definition, 
% $\propassign(\bigwedge^{k-1}_{j=1}\psi_j)\in \propneigh_i(w)$   and 
%  $\propassign(\psi_k)\not\in \propneigh_i(w)$.
%%Using the same argument of Lemma 3.1 in~\cite{Var2}, it follows that 
%So,
%   $\propassign(\bigwedge^{k-1}_{j=1}\psi_j)\neq \propassign(\psi_k)$.
%Then, %it is easy to see that 
%there 
%   is a world $u$ in the symmetrical difference of these sets 
%   such that $\propmodel,u\models (\bigwedge^{k-1}_{j=1}\psi_j\wedge\neg\psi_k)\vee(\neg(\bigwedge^{k-1}_{j=1}\psi_j)\wedge\psi_k)$. 
%   
%%Assume  $\B_i\psi_1, \dots, \B_i\psi_k$ are in 
%%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_j)=1$ for all $1\leq j < k$, and 
%%$\valuation(\B_i\psi_k)=0$.
%%By definition, $(\B_i \psi_1 \wedge \ldots \wedge \B_i \psi_{k-1})\rightarrow \B_i %(\psi_1\wedge \ldots \wedge \psi_{k-1})$ holds in $\EC^{n}$ models.
%%\nb{add this def somewhere} 
%%This means that $\valuation(\B_i(\bigwedge^{k-1}_{j=1}\psi_j))=1$.
%
%($\Leftarrow$) Suppose there is a $\varphi$-consistent valuation $\nu$ for $\prop{\varphi}$ such that 
%%there is   a $\varphi$-consistent valuation \valuation 
%%for $\prop{\varphi}$ such that 
%if $\B_i\psi_1, \dots, \B_i\psi_k$ are in 
%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_j)=1$ for all $1\leq j < k$, and 
%$\valuation(\B_i\psi_k)=0$, then 
%there is a $\varphi$-consistent $\EC^{n}$ model $$\propmodel_{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k}=(\propdomain_{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k},\{ \propneigh_{{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k}_{i}} \}_{i \in I},\propassign_{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k})$$ and a world 
%$w_{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k}\in \propdomain_{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k}$ such that 
%$$\propmodel_{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k}, w_{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k}\models ((\bigwedge^{k-1}_{j=1}\psi_j)\wedge\neg\psi_k)\vee(\neg(\bigwedge^{k-1}_{j=1}\psi_j)\wedge\psi_k).$$ 
%
%%either $(\bigwedge^{k-1}_{j=1}\psi_j\wedge\neg\psi_k)$ or 
%%$(\neg\psi_j\wedge\psi_k)$ for some $1\leq j < k$
%%is satisfied in a $\varphi$-consistent $\EC^{n}$ %\nb{check macro}
%% model. 
%% if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%%$\valuation(\B_i\psi_2)=0$, then 
%%there is a model $\propmodel_{\psi_1,\psi_2}=(\propdomain_{\psi_1,\psi_2},
%%\{ \propneigh_{{\psi_1,\psi_2}_{i}} \}_{i \in I},\propassign_{\psi_1,\psi_2})$
%% and a world 
%%$w_{\psi_1,\psi_2}\in \propdomain_{\psi_1,\psi_2}$ such that 
%%$\propmodel_{\psi_1,\psi_2}, w_{\psi_1,\psi_2}\models (\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$. 
%Let $\propmodel_1,\ldots,\propmodel_m$ be an enumeration of the models 
%$\propmodel_{\bigwedge^{k-1}_{j=1}\psi_j,\psi_k}$, as above.  That is, we take one model $\propmodel_{\bigwedge^{k-1}_{l=1}\psi_l,\psi_k}$ for each 
%pair $j=\bigwedge^{k-1}_{l=1}\psi_l,\psi_k$ 
%where $\propmodel_j = (\propdomain_j, \{ \propneigh_{j_{i}} \}_{i \in I},\propassign_j)$, 
%and let $w_1,\ldots,w_m$ be an enumeration of the worlds
% $w_{\bigwedge^{k-1}_{l=1}\psi_l,\psi_k}$, 
%with $j=\bigwedge^{k-1}_{l=1}\psi_l,\psi_k$ and  $w_j\in \propdomain_j$. We assume without loss of generality that $\propdomain_j\cap \propdomain_k=\emptyset$ 
%for $j\neq k$. 
%
%In the following, we define a $\varphi$-consistent $\EC^{n}$ model   $\propmodel = (\propdomain,\{ \propneigh_{i} \}_{i \in I}, \propassign)$ 
%for $\prop{\varphi}$. 
%Intuitively, we construct $\propmodel$ by taking the union of each 
%$\propmodel_j$ with the addition of a new world $w$ that 
%will satisfy $\prop{\varphi}$. 
%We define $\propdomain$ as $\bigcup_{1\leq j\leq n}\propdomain_j\cup \{w\}$, 
%where $w$ is fresh.
%%The tricky part of the proof is to define the assignment $\propassign$. 
%Before defining $\propneigh_{i}$ and $\propassign$, we define the function $J: {\sf sub}(\prop{\varphi})\rightarrow 2^{\Wmc}$
%with $J(\psi)=\bigcup_{0\leq j \leq m} \Vmc_j(\psi)$ for all $\psi\in {\sf sub}(\prop{\varphi})$, where %$I_i$ is as above for $1\leq i\leq n$, 
% %and
%$\Vmc_0: {\sf sub}(\varphi)\rightarrow  2^{\{w\}}$ is the function
%that assigns $\psi$ to $\{w\}$, if $\nu(\psi)=1$, 
%and to $\emptyset$, otherwise ($\Vmc_j$, for $1\leq j\leq m$, is as above).
%By construction, we have that $J(\neg \psi)=\propdomain\setminus J(\psi)$
%and $J(\psi_1\wedge \psi_2)=J(\psi_1)\cap J(\psi_2)$. 
%We define the assignment $\propassign$ as the function 
%$\propassign: \NPr(\varphi)\rightarrow 2^{\Wmc}$ satisfying 
% $\propassign(p_\elaxiom)=J(p_\elaxiom)$ for all $p_\elaxiom\in \NPr(\varphi)$. 
% 
%It remains to define $\propneigh_i$, for
%$i \in I$.
%%$1 \leq i \leq n$. 
%For $u\in \propdomain_j$ we first put $\alpha \subseteq W$ in $\propneigh_i(u)$ 
%precisely when 
%%\begin{itemize}
%%\item 
%$\propmodel_j,u \models \B_i \psi_\alpha$ and $\alpha = J(\psi_\alpha)$
%for some $\B_i\psi_\alpha \in {\sf sub}(\varphi)$.
%Then, we close $\propneigh_i$ under intersection so that $\propmodel$ is a $\EC^{n}$ model. The next two claims establish that $\propneigh_i$ is as expected.
%%; and
%%\item 
%%\end{itemize}
%%We claim that 
%\begin{claim}
%If $\beta \in \Nmc_i(u)$ and $\beta = J(\psi)$ for some $\B_i\psi\in{\sf sub}(\prop{\varphi})$,
%then $\propmodel_j,u\models\B_i\psi$.
%\end{claim}
%Indeed, since $\beta = J(\psi)\in \Nmc_i(u)$, 
%we must have that $\propmodel_j,u\models \B_i\psi_{1,\beta}$, \ldots, 
%$\propmodel_j,u\models \B_i\psi_{m,\beta}$ and  $\beta = \bigcap^{m}_{l=1} J(\psi_{l,\beta})$ for 
%some $\B_i\psi_{1,\beta}, \ldots, \B_i\psi_{m,\beta} \in{\sf sub}(\prop{\varphi})$. %
%Since $\propneigh_i$ is closed under intersection,
%in fact, we have that $\propmodel_j,u \models \B_i (\bigwedge^m_{l=1}\psi_{l,\beta})$.
%%\nb{intersection}
%But since
%$J(\psi)=\bigcap^{m}_{i=1} J(\psi_{i,\beta})$, we also have $\propassign_j(\psi)=\bigcap^{m}_{l=1}\propassign_j(\psi_{l,\beta})$ 
%(recall that $\propdomain_j \cap \propdomain_k = \emptyset$ for  
%$k \neq j$), so $\propmodel_j,u\models \B_i\psi$ iff 
%$\propmodel_j,u \models \B_i (\bigwedge^m_{l=1}\psi_{l,\beta})$.
%It follows that $\propmodel_j,u\models \B_i\psi$.
%
%\medskip
%
%Regarding the fresh 
%world $w$ introduced above in $\propdomain$,
%we first put $\alpha \subseteq \Wmc$ in $\propneigh_i(w)$   precisely 
%when $\nu(\B_i\psi_\alpha) = 1$ and $\alpha = J(\psi_\alpha)$ for some 
%$\B_i\psi_\alpha \in {\sf sub}(\prop{\varphi})$.
%Then, we again close $\propneigh_i$ under intersection so that $\propmodel$ is a $\EC^{n}$ model.
%%We claim that 
%\begin{claim}
%If 
%$\beta \in \propneigh_i(w)$ and $\beta = J(\bigwedge^{k-1}_{l=1}\psi_l)$ for some $\B_i \psi_1, \ldots, \B_i \psi_{k-1} \in{\sf sub}(\prop{\varphi})$ 
%then  $\valuation(\B_i\psi_l)=1$ for all $1\leq l < k$.
%\end{claim}
%Indeed, since $\beta = J(\bigwedge^{k-1}_{l=1}\psi_l)\in \propneigh_i(w)$ 
%we must have that $\nu(\B_i\psi_{1,\beta})=1, \ldots, \nu(\B_i\psi_{m,\beta})=1$ and 
%$\beta = \bigcap^{m}_{i=1} J(\psi_{i,\beta})$ for some 
%$\B_i\psi_{1,\beta}, \ldots, \B_i\psi_{m,\beta} \in{\sf sub}(\prop{\varphi})$. %\nb{intersection}
%Suppose now that $\nu(\bigwedge^{k-1}_{l=1}\psi_l) = 0$. Then, by assumption, there exists a structure
%$\propmodel_j = (\propdomain_j, \{ \propneigh_{j_i} \}_{i \in I}, \propassign_j)$ and a world $w_j
%\in \propdomain_j$ such that $\propmodel_j,w_j \models (\bigwedge^{k-1}_{l=1}\psi_{l,\beta} \wedge \neg(\bigwedge^{k-1}_{l=1}\psi_l))\vee(\neg(\bigwedge^{k-1}_{l=1}\psi_{l,\beta}) \wedge (\bigwedge^{k-1}_{l=1}\psi_l))$. 
%It follows that $\propassign_j(\bigwedge^{k-1}_{l=1}\psi_{l,\beta})\neq \propassign_j(\bigwedge^{k-1}_{l=1}\psi_l)$. 
%Consequently $J(\bigwedge^{k-1}_{l=1}\psi_{l,\beta})\neq J(\bigwedge^{k-1}_{l=1}\psi_l)$, which is a contradiction.  
%%\nb{O :... talk about consistent}
%
%\medskip
%
%We now show by induction on the structure of formulas 
%that $\propassign$ and $J$ agree on ${\sf sub}(\prop{\varphi})$. 
%This holds by construction for atomic propositions. It is easy to deal 
%with propositional connectives, since we know that $J(\neg \psi)=\propdomain\setminus J(\neg \psi)$
%and  $J(\psi_1\wedge \psi_2)=J(\psi_1)\cap J(\psi_2)$ 
%and similarly for $\propassign$. Assume inductively that $\propassign(\psi) = J(\psi)$.
%Suppose first that $u\in J(\B_i\psi)$. Then, either $u=w$ and $\nu(\B_i\psi)=1$
%or $u\in \propdomain_j$ and $\propmodel_j,u\models\B_i\psi$. In either case 
%we have that $J(\psi)\in \propneigh_i(u)$. Since 
%$\propassign(\psi) = J(\psi)$, it follows that $\propmodel,u\models \B_i\psi$, 
%that is, $u\in \propassign(\B_i\psi)$. Suppose now that $u\in \propassign(\B_i\psi)$, 
%that is, $\propmodel,u\models \B_i\psi$, or, equivalently, $\propassign(\psi)\in \propneigh_i(u)$.
%Since $\propassign(\psi) = J(\psi)$ it follows that either $u=w$ and 
%$\nu(\B_i\psi)=1$ or $u\in \propdomain_j$ and $\propmodel_j,u\models \B_i\psi$. 
%In either case we have that $u\in J(\B_i\psi)$. 
%
%Since $\nu(\prop{\varphi})=1$, we have that $w\in J(\prop{\varphi})$, 
%and consequently $w\in \propassign(\prop{\varphi})$. That 
%is, $\propmodel,w\models\prop{\varphi}$. 
%The fact that $\propmodel$ is a $\EC^{n}$ model follows 
%from the definition of $\propneigh_i$.
%The fact that $\propmodel$ is a $\varphi$-consistent  model follows from 
%the fact that $\nu$, used to construct the assignment 
%related to $w$, is $\varphi$-consistent and 
%the models $\propmodel_1,\ldots,\propmodel_m$, used to define 
%the remaining worlds in $\Wmc$, are all $\varphi$-consistent %$\EC^{n}$ 
%models. 
%%Now the lemma follows from Lemma~\ref{lem:general}.
%%Take $\bigwedge^{k-1}_{j=1}\psi_j$ as $\psi'$
%\end{proof}
%
%
%
%\begin{restatable}{lemma}{LemmapropN}\label{lem:proplemmaN}
%A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\EN^{n}$ model
%iff
%%if, and only if,
%there is   a $\varphi$-consistent valuation \valuation 
%for $\prop{\varphi}$ such that 
%\begin{enumerate}
%\item if $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and
%$\valuation(\B_i\psi)=0$, then $\neg \psi$ 
%is satisfied in a $\varphi$-consistent $\EN^{n}$ model; %and 
%\item if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%$\valuation(\B_i\psi_2)=0$, then $(\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$
%is satisfied in a $\varphi$-consistent $\EN^{n}$ model. 
%\end{enumerate}
%\end{restatable}
%%
%\begin{proof}%[Sketch]
%We start with proving ($\Rightarrow$). 
%Suppose that $\prop{\varphi}$ is satisfied in a world $w$ of a $\varphi$-consistent $\EN^{n}$ model 
% $\propmodel = (\propdomain, \{ \propneigh_{i} \}_{i \in I}, \propassign)$. That is, 
% $\propmodel, w\models \prop{\varphi}$. We define a $\varphi$-consistent valuation for 
% $\prop{\varphi}$
% by setting $\nu(\psi)=1$ if $\propmodel, w\models \psi$ and $\nu(\psi) = 0$
% if  $\propmodel, w\not\models \psi$. 
% It is easy to check that $\nu$ is indeed a 
% $\varphi$-consistent valuation (given that $\propmodel$ is a  
% $\varphi$-consistent $\EN^{n}$ model). 
%
%\textit{Point 1.}
%%\paragraph{Point 1}
%By definition,  $\B_i {\sf true}$ holds in $\EN^{n}$ models. %\nb{add this def somewhere}
%Since there is a valuation $\valuation$ such that 
%$\valuation(\B_i\psi)=0$ we have that
%$\psi$ cannot be true in all valuations (otherwise
%$\psi\equiv {\sf true}$ would hold and  $\valuation$ 
%would violate %validity of 
%$\B_i {\sf true}$ in $\EN^{n}$ models).
%This means that 
%%We have that
% $\neg \psi$ is 
%$\EN^{n}$  satisfiable.
%
%\textit{Point 2.}
%%\paragraph{Point 2}
%Assume that 
% $\B_i\psi_1$ and $\B_i\psi_2$ are in ${\sf sub}(\prop{\varphi})$, 
% $\nu(\B_i\psi_1)=1$ and $\nu(\B_i\psi_2)=0$. Then $\propmodel,w\models \B_i\psi_1$
% and $\propmodel,w\not\models \B_i\psi_2$. Thus, by definition, 
% $\propassign(\psi_1)\in \propneigh_i(w)$ and 
%  $\propassign(\psi_2)\not\in \propneigh_i(w)$.
%%Using the same argument of Lemma 3.1 in~\cite{Var2}, it follows that 
%So,
%   $\propassign(\psi_1)\neq \propassign(\psi_2)$.
%Then, %it is easy to see that 
%there 
%   is a world $u$ in the symmetrical difference of these sets 
%   such that $\propmodel,u\models (\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$. 
%   
%%\medskip
%
%The proof of the converse ($\Leftarrow$)
%%for  the second bullet point 
%is as follows. %in Lemma~\ref{lem:general}.
%%It holds in $\EC^{n}$ models because $\B_i {\sf true}$
% Suppose there is a $\varphi$-consistent valuation $\nu$ for $\prop{\varphi}$ such that 
% Point~1
%%\textbf{Point 1}
%and
%Point~2
%%\textbf{Point 2}
%hold. 
%That is, 
%\begin{itemize}
%\item if $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and
%$\valuation(\B_i\psi)=0$ then 
%there is a $\varphi$-consistent $\EN^{n}$ model $\propmodel_{\psi}=(\propdomain_{\psi},
%\{ \propneigh_{{\psi}_{i}} \}_{i \in I},\propassign_{\psi})$
%%
% and a world 
%$w_{\psi}\in \propdomain_{\psi}$ such that 
%$\propmodel_{\psi}, w_{\psi}\models \neg\psi$; and 
%%$\neg \psi$ is 
%%$\EN^{n}$ satisfiable; and
%\item if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%$\valuation(\B_i\psi_2)=0$, then 
%there is a $\varphi$-consistent $\EN^{n}$ model $\propmodel_{\psi_1,\psi_2}=(\propdomain_{\psi_1,\psi_2},
%\{ \propneigh_{{\psi_1,\psi_2}_{i}} \}_{i \in I},\propassign_{\psi_1,\psi_2})$
%%
% and a world 
%$w_{\psi_1,\psi_2}\in \propdomain_{\psi_1,\psi_2}$ such that 
%$\propmodel_{\psi_1,\psi_2}, w_{\psi_1,\psi_2}\models (\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$. 
%\end{itemize}
%Let $\propmodel_1,\ldots,\propmodel_m$ be an enumeration of $\EN^{n}$ models 
%$\propmodel_{\psi}$ and $\propmodel_{\psi_1,\psi_2}$, as above.  That is, we take one model $\propmodel_{\psi}$ and one model $\propmodel_{\psi_1,\psi_2}$ for each such
%subformula $j=\psi$ and pair of subformulas $j=\psi_1,\psi_2$ where $\propmodel_j = (\propdomain_j, \{ \propneigh_{j_{i}} \}_{i \in I},\propassign_j)$, 
%and let $w_1,\ldots,w_m$ be an enumeration of the worlds $w_{\psi}$ and $w_{\psi_1,\psi_2}$, 
%with $w_j\in \propdomain_j$. Assume without loss of generality that $\propdomain_j\cap \propdomain_k=\emptyset$ 
%for $j\neq k$. 
%%
%In the following, we define a $\varphi$-consistent $\EN^{n}$ model   $\propmodel = (\propdomain,\{ \propneigh_{i} \}_{i \in I}, \propassign)$ 
%for $\prop{\varphi}$. 
%
%Intuitively, we construct $\propmodel$ by taking the union of each 
%$\propmodel_j$ with the addition of a new world $w$ that 
%will satisfy $\prop{\varphi}$. 
%We define $\propdomain$ as $\bigcup_{1\leq j\leq n}\propdomain_j\cup \{w\}$, 
%where $w$ is fresh.
%%The tricky part of the proof is to define the assignment $\propassign$. 
%Before defining $\propneigh_{i}$ and $\propassign$, we define the function $J: {\sf sub}(\prop{\varphi})\rightarrow 2^{\Wmc}$
%with $J(\psi)=\bigcup_{0\leq j \leq m} \Vmc_j(\psi)$ for all $\psi\in {\sf sub}(\prop{\varphi})$, where %$I_i$ is as above for $1\leq i\leq n$, 
% %and
%$\Vmc_0: {\sf sub}(\prop{\varphi})\rightarrow  2^{\{w\}}$ is the function
%that assigns $\psi$ to $\{w\}$, if $\nu(\psi)=1$, 
%and to $\emptyset$, otherwise ($\Vmc_j$, for $1\leq j\leq m$, is as above).
%By construction, we have that $J(\neg \psi)=\propdomain\setminus J(\psi)$
%and $J(\psi_1\wedge \psi_2)=J(\psi_1)\cap J(\psi_2)$. 
%We define the assignment $\propassign$ as the function 
%$\propassign: \NPr(\varphi)\rightarrow 2^{\Wmc}$ satisfying 
% $\propassign(p_\elaxiom)=J(p_\elaxiom)$ for all $p_\elaxiom\in \NPr(\varphi)$. 
% 
%It remains to define $\propneigh_i$,
%for
%$i \in I$.
%%$1 \leq i \leq n$. 
%For $u\in \propdomain_j$ we put  $\alpha \subseteq \Wmc$ in $\propneigh_i(u)$ 
%precisely when $\alpha=\Wmc$, or, $\alpha = J(\psi_{\alpha})$ and
%$\propmodel_j,u \models \B_i \psi_{\alpha}$,  
%for some $\B_i\psi_{\alpha} \in {\sf sub}(\prop{\varphi})$.
%The next two claims establish that $\propneigh_i$ is as expected. 
%%We claim that 
%\begin{claim}
%If $\beta \in \Nmc_i(u)$ and $\beta = J(\psi)$ for some $\B_i\psi\in{\sf sub}(\prop{\varphi})$,
%then $\propmodel_j,u\models\B_i\psi$.
%\end{claim}
%\begin{proof}[Proof of Claim]
%Indeed, since $\beta = J(\psi)\in \Nmc_i(u)$, 
%we must have that either $\beta=\Wmc$ or $\propmodel_j,u\models \B_i\psi_{\beta}$ and  $\beta = J(\psi_{\beta})$ for 
%some $\B_i\psi_\beta \in{\sf sub}(\prop{\varphi})$.
%In the former case, as all $\propmodel_j$ models are $\EN^{n}$ models, 
%we have that $\propmodel_j,u\models \B_i\psi$.
%% (in this case, $\psi$
%%is true in all worlds in all $\EN^{n}$ models).
%In the latter,  since
%$J(\psi)=J(\psi_\beta)$, we also have $\propassign_j(\psi)=\propassign_j(\psi_\beta)$ 
%(recall that $\propdomain_j \cap \propdomain_k = \emptyset$ for  
%$k \neq j$), so $\propmodel_j,u\models \B_i\psi$ iff 
%$\propmodel_j,u \models \B_i \psi_\beta$.
%It follows that $\propmodel_j,u\models \B_i\psi$.
%\end{proof}
%
%Also, we put $\alpha \subseteq \Wmc$ in $\propneigh_i(w)$ (recall $w$ is the fresh 
%world introduced above in $\propdomain$) precisely 
%when $\alpha = \Wmc$ or $\nu(\B_i\psi_\alpha) = 1$ and $\alpha = J(\psi_\alpha)$ for some 
%$\B_i\psi_\alpha \in {\sf sub}(\prop{\varphi})$.
%
%\begin{claim}
%If 
%$\beta \in \propneigh_i(w)$ and $\beta = J(\psi)$ for some $\B_i \psi \in{\sf sub}(\prop{\varphi})$ 
%then $\nu(\B_i \psi) = 1$.
%\end{claim}
%\begin{proof}[Proof of Claim]
%Indeed, since $\beta = J(\psi)\in \propneigh_i(w)$ 
%we must have that either $\beta=\Wmc$
%or $\nu(\B_i\psi_\beta)=1$ and $\beta = J(\psi_\beta)$ for some 
%$\B_i\psi_\beta \in{\sf sub}(\prop{\varphi})$. 
%Suppose  that $\nu(\B_i\psi) = 0$ and $\beta\neq\Wmc$.
%Then, by assumption, there exists a $\varphi$-consistent $\EN^{n}$ model
%$\propmodel_j = (\propdomain_j, \{ \propneigh_{j_i} \}_{i \in I}, \propassign_j)$ and a world $w_j
%\in \propdomain_j$ such that $\propmodel_j,w_j \models (\psi_\beta \wedge \neg\psi)\vee(\neg\psi_\beta \wedge \psi)$. 
%It follows that $\propassign_j(\psi_\beta)\neq \propassign_j(\psi)$. 
%Consequently $J(\psi_\beta)\neq J(\psi)$, which is a contradiction.  
%Now, suppose   that $\nu(\B_i\psi) = 0$ and $\beta=\Wmc$.
%By assumption,
%%$\neg \psi$ is  satisfiable in a $\varphi$-consistent $\EN^{n}$ model.
%%This means that 
%there exists a $\varphi$-consistent $\EN^{n}$ model
%$\propmodel_j = (\propdomain_j, \{ \propneigh_{j_i} \}_{i \in I}, \propassign_j)$ and a world $w_j
%\in \propdomain_j$ such that $\propmodel_j,w_j \models \neg\psi$.
%It follows that $\propassign_j(\psi)\neq \Wmc$. Consequently $\beta= J(\psi)\neq \Wmc$, which is a contradiction.  Then,  $\nu(\B_i \psi) = 1$, as required.
%%\nb{changing}
%%, which means that
%%$\beta=\Wmc$.
%%\nb{O :... talk about consistent}
%\end{proof}
%
%We now show by induction on the structure of formulas 
%that $\propassign$ and $J$ agree on ${\sf sub}(\prop{\varphi})$. 
%This holds by construction for atomic propositions. It is easy to deal 
%with propositional connectives, since we know that $J(\neg \psi)=\propdomain\setminus J(\neg \psi)$
%and  $J(\psi_1\wedge \psi_2)=J(\psi_1)\cap J(\psi_2)$ 
%and similarly for $\propassign$. Assume inductively that $\propassign(\psi) = J(\psi)$.
%Suppose first that $u\in J(\B_i\psi)$. Then, either $u=w$ and $\nu(\B_i\psi)=1$
%or $u\in \propdomain_j$ and $\propmodel_j,u\models\B_i\psi$. In either case 
%we have that $J(\psi)\in \propneigh_i(u)$. Since 
%$\propassign(\psi) = J(\psi)$, it follows that $\propmodel,u\models \B_i\psi$, 
%that is, $u\in \propassign(\B_i\psi)$. Suppose now that $u\in \propassign(\B_i\psi)$, 
%that is, $\propmodel,u\models \B_i\psi$, or, equivalently, $\propassign(\psi)\in \propneigh_i(u)$.
%Since $\propassign(\psi) = J(\psi)$ it follows that either $u=w$ and 
%$\nu(\B_i\psi)=1$ or $u\in \propdomain_j$ and $\propmodel_j,u\models \B_i\psi$. 
%In either case we have that $u\in J(\B_i\psi)$. 
%
%Since $\nu(\prop{\varphi})=1$, we have that $w\in J(\prop{\varphi})$, 
%and consequently $w\in \propassign(\prop{\varphi})$. That 
%is, $\propmodel,w\models\prop{\varphi}$. 
%The fact that $\propmodel$ is $\varphi$-consistent follows from 
%the fact that $\nu$, used to construct the assignment 
%related to $w$, is $\varphi$-consistent and 
%the models $\propmodel_1,\ldots,\propmodel_m$, used to define 
%the remaining worlds in $\Wmc$, are all $\varphi$-consistent.
%The fact that  $\propmodel$ contains the unit is by construction, that is,
%we defined $\propmodel$
%%. That is, 
%so that for all 
%$i\in [1,n]$ and all $w\in\Wmc$, we have that $\Wmc\in\Nmc_i(w)$. 
%Thus, $\propmodel$ is a $\varphi$-consistent $\EN^{n}$ model that satisfies 
%$\prop{\varphi}$, as required. 
%\end{proof}
%
%
%
%To determine satisfiability of $\prop{\varphi}$ in a $\varphi$-consistent model, we use Lemma~\ref{lem:prop} and the characterizations above. 
%To establish complexity results, %for the upper bound of $\CALCg$, 
%we use the fact that there are only quadratically many   subformulas in $\prop{\varphi}$. 
%Satisfiability in
%\ALC is \ExpTime-complete  and so, one can determine in exponential time
%whether a valuation is $\varphi$-consistent. For an \ExpTime~upper bound, one can
%deterministically compute all possible $\varphi$-consistent valuations for 
%$(\bigwedge^{k-1}_{j=1}\psi_j\wedge\neg\psi_k)$ (or $(\psi_1 \wedge \neg \psi_2)$) and
%decide satisfiability of $\prop{\varphi}$ by a $\varphi$-consistent model using a bottom-up strategy (as in~\cite{Baader:2012:LOD:2287718.2287721}). Since satisfiability in \ALC is \ExpTime-hard, our upper bound is tight.
%
%\begin{theorem}
%The $\CALCg$ and $\NALCg$ formula satisfiability problems on constant domain neighbourhood models are \ExpTime-complete.
%%Satisfiability in  $\CALCg$  and $\NALCg$ is \ExpTime-complete.
%\end{theorem}
%
%\begin{restatable}{lemma}{LemmapropP}\label{lem:proplemmaP}
%	A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\EP^{n}$ model
%	iff
%	%if, and only if,
%	there is   a $\varphi$-consistent valuation \valuation 
%	for $\prop{\varphi}$ such that 
%	\begin{enumerate}
%		\item if $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and
%		$\valuation(\B_i\psi)=1$, then $\psi$ 
%		is satisfied in a $\varphi$-consistent $\EP^{n}$ model; %and 
%		\item if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%		${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%		$\valuation(\B_i\psi_2)=0$, then $(\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$
%		is satisfied in a $\varphi$-consistent $\EP^{n}$ model. 
%	\end{enumerate}
%\end{restatable}
%
%\begin{restatable}{lemma}{LemmapropQ}\label{lem:proplemmaQ}
%	A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\EQ^{n}$ model
%	iff
%	%if, and only if,
%	there is   a $\varphi$-consistent valuation \valuation 
%	for $\prop{\varphi}$ such that 
%	\begin{enumerate}
%		\item if $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and
%		$\valuation(\B_i\psi)=1$, then $\neg\psi$ 
%		is satisfied in a $\varphi$-consistent $\EQ^{n}$ model; %and 
%		\item if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%		${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%		$\valuation(\B_i\psi_2)=0$, then $(\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$
%		is satisfied in a $\varphi$-consistent $\EQ^{n}$ model. 
%	\end{enumerate}
%\end{restatable}
%
%\begin{restatable}{lemma}{LemmapropD}\label{lem:proplemmaD}
%	A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\ED^{n}$ model
%	iff
%	%if, and only if,
%	there is   a $\varphi$-consistent valuation \valuation 
%	for $\prop{\varphi}$ such that 
%	\begin{enumerate}
%		\item if $\B_i\psi_1$ and $\B_i\psi_2$ are in ${\sf sub}(\prop{\varphi})$,
%		$\valuation(\B_i\psi_1)=1$ and $\valuation(\B_i\psi_2)=1$, then
%		$(\psi_1\wedge\psi_2)\vee(\neg\psi_1\wedge\neg\psi_2)$   
%		is satisfied in a $\varphi$-consistent $\ED^{n}$ model; %and 
%		\item if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%		${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%		$\valuation(\B_i\psi_2)=0$, then $(\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$
%		is satisfied in a $\varphi$-consistent $\ED^{n}$ model. 
%	\end{enumerate}
%\end{restatable}
%
%\begin{restatable}{lemma}{LemmapropT}\label{lem:proplemmaT}
%	A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\ET^{n}$ model
%	iff
%	%if, and only if,
%	there is   a $\varphi$-consistent valuation \valuation 
%	for $\prop{\varphi}$ such that 
%	\begin{enumerate}
%		\item if $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and 
%		$\valuation(\B_i\psi)=1$   then
%		$\psi$   \todo{to check}
%		is satisfied in a $\varphi$-consistent $\ET^{n}$ model; %and 
%		\item if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%		${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and 
%		$\valuation(\B_i\psi_2)=0$, then $(\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$
%		is satisfied in a $\varphi$-consistent $\ET^{n}$ model. 
%	\end{enumerate}
%\end{restatable}
%%\begin{restatable}{lemma}{LemmapropCMN}\label{lem:proplemmaCMN}
%%	A formula $\prop{\varphi}$ is satisfied in a $\varphi$-consistent $\EMCN^{n}$ model
%%	iff
%%	%if, and only if,
%%	there is   a $\varphi$-consistent valuation \valuation 
%%	for $\prop{\varphi}$ such that 
%%	%\begin{enumerate}
%%		%\item 
%%		if $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and
%%		$\valuation(\B_i\psi)=0$, then both $\bigwedge_{\valuation(\B_i\psi')=1}  \B_i\psi'\wedge\neg\psi$ and $\bigwedge_{\valuation(\B_i\psi')=1}  \psi'\wedge\neg\psi $
%%		are satisfied in a $\varphi$-consistent $\EMCN^{n}$ model. %; %and 
%%	%	\item if $\B_i\psi_1$ and $\B_i\psi_2$ are in 
%%%		${\sf sub}(\prop{\varphi})$, $\valuation(\B_i\psi_1)=1$, and %
%%%		$\valuation(\B_i\psi_2)=0$, then $(\psi_1\wedge\neg\psi_2)\vee(\neg\psi_1\wedge\psi_2)$
%%%		is satisfied in a $\varphi$-consistent $\EMCN^{n}$ model. 
%%	%\end{enumerate}
%%\end{restatable}
%%\begin{proof} 
%%($\Rightarrow$) Suppose that $\prop{\varphi}$ is satisfied in a world $w$ of a $\varphi$-consistent $\EMCN^{n}$ model 
%%$\propmodel = (\propdomain, \{ \propneigh_{i} \}_{i \in I}, \propassign)$. That is, 
%%$\propmodel, w\models \prop{\varphi}$. We define a $\varphi$-consistent valuation for 
%%$\prop{\varphi}$
%%by setting $\nu(\psi)=1$ if $\propmodel, w\models \psi$ and $\nu(\psi) = 0$
%%if  $\propmodel, w\not\models \psi$. 
%%It is easy to check that $\nu$ is indeed a 
%%$\varphi$-consistent valuation (given that $\propmodel$ is a  
%%$\varphi$-consistent $\EMCN^{n}$ model). \nb{Ana: to check}
%%Assume   $\B_i\psi$ is in ${\sf sub}(\prop{\varphi})$ and
%%$\valuation(\B_i\psi)=0$.
%%%
%%Then %$\propmodel,w\models \B_i\psi_j$ for all $1\leq j < k$,
%%%and 
%%$\propmodel,w\not\models \B_i\psi$.
%%By necessitation in $\EMCN^{n}$ models, $\propmodel,w\not\models \psi$.
%%So $\propmodel,w\models \neg\psi$.
%%By definition, $\propmodel,w\models \B_i\psi'$ when $\valuation(\B_i\psi')=1$.
%%This means that $\bigwedge_{\valuation(\B_i\psi')=1}  \B_i\psi'\wedge\neg\psi$ is  satisfied in a $\varphi$-consistent $\EMCN^{n}$ model.
%%%So $\propmodel,w\models \B_i (\psi_1\wedge \ldots \wedge \psi_{k-1})$ 
%%%and $\propmodel,w\not\models \B_i\psi_k$.
%%%This means that $\valuation(\B_i(\bigwedge^{k-1}_{j=1}\psi_j))=1$
%%%while $\valuation(\B_i\psi_k)=0$.
%%%
%%
%%We now argue about $\bigwedge_{\valuation(\B_i\psi')=1}  \psi'\wedge\neg\psi $. \nb{Ana: on going}
%%By definition, 
%%$\propassign(\bigwedge_{\valuation(\B_i\psi')=1}\psi')\in \propneigh_i(w)$   and 
%%$\propassign(\psi)\not\in \propneigh_i(w)$.
%%%Using the same argument of Lemma 3.1 in~\cite{Var2}, it follows that 
%%So,
%%$\propassign(\bigwedge^{k-1}_{j=1}\psi_j)\neq \propassign(\psi_k)$.
%%Then, %it is easy to see that 
%%there 
%%is a world $u$ in the symmetrical difference of these sets 
%%such that $\propmodel,u\models (\bigwedge_{\valuation(\B_i\psi')=1}\psi'\wedge\neg\psi)\vee(\neg(\bigwedge_{\valuation(\B_i\psi')=1}\psi')\wedge\psi)$.  
%%\end{proof}
%
%
%%\subsection{{\color{red}{Unified ``Vardi's lemma'' for all logics}}}
%
%
%
%
%
%\newpage

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Applications and Extensions}
%
%\subsection{Somebody Knows}
